From Intervention to Domain Transportation: A Novel Perspective to Optimize Recommendation

The interventional nature of recommendation has attracted increasing attention in recent years. It particularly motivates researchers to formulate learning and evaluating recommendation as causal inference and data missing-not-at-random problems. However, few take seriously the consequence of violating the critical assumption of overlapping, which we prove can significantly threaten the validity and interpretation of the outcome. We find a critical piece missing in the current understanding of information retrieval (IR) systems: as interventions, recommendation not only affects the already observed data, but it also interferes with the target domain (distribution) of interest. We then rephrase optimizing recommendation as finding an intervention that best transports the patterns it learns from the observed domain to its intervention domain. Towards this end, we use domain transportation to characterize the learning-intervention mechanism of recommendation. We design a principled transportation-constraint risk minimization objective and convert it to a two-player minimax game. We prove the consistency, generalization, and excessive risk bounds for the proposed objective, and elaborate how they compare to the current results. Finally, we carry out extensive real-data and semi-synthetic experiments to demonstrate the advantage of our approach, and launch online testing with a real-world IR system.

==> implementation.tex <==
\begin{algorithm}[H]
\label{algo:minimax}
\caption{Batch-wise GDA for Minimax Optimization}
\KwIn{$\tilde{\Dcal}(t)$: a batch of training sample of size $m$ at step $t$. $\eta$: the learning rate for ascent step. $\gamma$: shrinking parameter for the learning rate of descent step. $\lambda$: the regularization parameter.}
\For{each step $t=0,1,\ldots$}{
Compute $\text{reco}(u,i;f_{\theta_1})$ for $(u,i)\in\tilde{\Dcal}(t)$ (see Section \ref{sec:experiment} for the computation detail)\;
$\thetabf_1^{(t+1)} \leftarrow \thetabf_1^{(t)} - \frac{\eta}{\gamma} \nabla_{\thetabf_1} \Lcal_{\lambda}\big([\thetabf_1^{(t)}, \thetabf_2^{(t)}], \thetabf_3^{(t)}\big)$; $\thetabf_2^{(t+1)} \leftarrow \thetabf_2^{(t)} - \frac{\eta}{\gamma} \nabla_{\thetabf_2} \Lcal_{\gamma}\big([\thetabf_1^{(t)}, \thetabf_2^{(t)}], \thetabf_3^{(t)}\big)$\;
$\thetabf_3^{(t+1)} \leftarrow \thetabf_3^{(t)} + \eta \nabla_{\thetabf_3} \Lcal_{\lambda}\big([\thetabf_1^{(t)}, \thetabf_2^{(t)}], \thetabf_3^{(t)}\big)$.
}
\end{algorithm}

The key to our implementation is by perceiving Wasserstein distance as a binary classification problem with Lipschitz-bounded classifier, as we discussed in Section \ref{sec:optimal-transport}. Towards this end, we denote by $g\in\Gcal$ (or $\Gcal_{\Phi}$ under the representation mapping) any suitable classifier for the computation of $d_W$. Without loss of generality, we let $w$, $f$ and $g$ be parameterized by $\thetabf_1$, $\thetabf_2$ and $\thetabf_3$ that may consists of the (shared) representations under $\Phi$. With (\ref{eqn:new-obj}), it is straightforward to verify that the optimization problem is exactly: $\min_{[\thetabf_1, \thetabf_2]}\max_{\thetabf_3} \Lcal_{\lambda}([\thetabf_1, \thetabf_2], \thetabf_3)$, with $\Lcal_{\lambda}$ given by:
\begin{equation}
\label{eqn:minimax-obj}
\sum_{(u,i)\in\Dcal} w_{ui}(\thetabf_2) \ell_{ui}\big(f_{\thetabf_1}\big) + \lambda \Big(\sum_{(u,i)\in\Dcal}w_{ui}(\thetabf_2) \cdot g_{ui}(\thetabf_3) - \sum_{(u,i)\in\Dcal} \text{reco}(u,i;f_{\thetabf_1}) \cdot g_{ui}(\thetabf_3) \Big).
\end{equation}

In the above minimax game, the first player optimizes $f$ and $w$ for both the training risk and the domain imbalance. Imagine $w_{ui} = \text{reco}(u,i;f)$ everywhere so $P_w$ and $P_f$ are fully balanced, then the regularization term equals to zero regardless of how the second player manipulate $g$. Obviously, this is unrealistic unless the empirical risk is minimized at the same time and $w_{ui}$ (assume to be in $(0,1)$) all hit the boundary value. 
% Otherwise, $g_{ui}$ can always be made larger on where $w_{ui}$ and $\text{reco}(u,i;f_{\theta_1})$ disagree the most, i.e. by exploiting the imbalance between $P_w$ and $P_f$ \qye{A bit wordy. What's the insight from the above sentences?}. 
% Assume for now that the global equilibrium is reached. Neither player will be able to change the objective without knowing each other's strategy, which means $f$ and $w$ cannot further improve the empirical risk and domain balance at the same time. It suggests we find the candidate $f$ who minimizes the empirical risk on the training domain that is most balanced with its deployment domain, which is achieved by the resulting $w$. We propose a two-time-scale gradient descent ascent (GDA) algorithm described in Algorithm \ref{algo:minimax}.
If the global equilibrium is reached, neither player can change the objective without knowing each other's strategy. It means $f$ and $w$ cannot improve the empirical risk and domain balance at the same time, so we find the $f$ who minimizes the empirical risk on the training domain that is most balanced with its deployment domain, which is achieved by the resulting $w$. We propose a two-time-scale gradient descent ascent (GDA) approach in Algorithm \ref{algo:minimax}, with its stability and convergence guarantees proved in Appendix ???. 


% By using bounded Lipschitz functions for $w_{\thetabf_1}$, $f_{\thetabf_2}$, we show in Appendix B that the gradient of $\Lcal_{\lambda}$ is $L-$Lipschitz.
% It is indicated by \cite{daskalakis2018limit} that GDA with $\eta \leq 1/L$ avoids unstable critical points for almost all initialization, which means that $\big(\thetabf_1^{(t}, \thetabf_2^{(t)}, \thetabf_3^{(t)}\big)$ is unlikely to cycle as $t$ grows. Furthermore, any stationary point yielded by GDA with large $\gamma$ is basically a \emph{local minimax point} except degenerated case \citep{jin2020local}, and thus the convergence guarantee of Algorithm \ref{algo:minimax}. Here, a solution $(\thetabf_1^*, \thetabf_2^*, \thetabf_3^*)$ is local minimax if there exits $\delta_0 > 0$ and a function $h$ satisfying $\lim_{\delta\rightarrow 0}h(\delta) \rightarrow 0$ such that $\forall \delta \in (0, \delta_0]$, and any $(\thetabf_1, \thetabf_2, \thetabf_3)$ satisfying $\big\Vert [\thetabf_1, \thetabf_2] - [\thetabf_1^*, \thetabf_2^*]\big\Vert_2 \leq \delta$ and $\Vert \thetabf_3 - \thetabf_3^* \Vert_2 \leq h(\delta)$, it holds that:
% \[
% \Lcal_{\lambda}\big([\thetabf_1^*, \thetabf_2^*], \thetabf_3\big) \leq \Lcal_{\lambda}\big([\thetabf_1^*, \thetabf_2^*], \thetabf_3^* \big) \leq \max_{\thetabf_3':\Vert \thetabf_3' - \thetabf_3^*\Vert_2 \leq h(\delta)}\Lcal_{\lambda}\big([\thetabf_1, \thetabf_2], \thetabf_3'\big).
% \]
% In other words, by using the two-time-scale GDA algorithm with a small $\eta$ and a large $\gamma$, our resulting solution has a similar role as a local minimum/maximum in a minimization/maximization problem --- the global Nash equilibrium, if any, must be one of the solutions yielded by the GDA in Algorithm \ref{algo:minimax}.


